Privacy and Integrity Preserving Training Using Trusted Hardware

Privacy and security-related concerns are growing as machine learning reaches diverse application domains. The data holders want to train with private data while exploiting accelerators, such as GPUs, that are hosted in the cloud. However, Cloud systems are vulnerable to attackers that compromise the privacy of data and integrity of computations. This work presents DarKnight, a framework for large DNN training while protecting input privacy and computation integrity. DarKnight relies on cooperative execution between trusted execution environments (TEE) and accelerators, where the TEE provides privacy and integrity verification, while accelerators perform the computation heavy linear algebraic operations.

==> 4.5Guarantee.tex <==
\section{Privacy Guarantee}
\label{sec:guarantee}
In this section, we bound the information that leaks, when using Darknight's blinding approach. 
In particular, we measure the amount of information the adversary can potentially gain about the raw data from the blinded data, if the adversary has access to an unlimited computation power. The amount of information leaked by $\bar{\mathbf x}^{(i)}$'s about $\mathbf x^{(1)},\dots,\mathbf x^{(K)}$ is the \textbf{mutual information (MI)} between these two sets of variables, defined by~\citep{cover1999elements}
\begin{align}
    I(\mathbf x^{(1)},\dots,\mathbf x^{(K)} ; \bar{\mathbf x}^{(1)},\dots,\bar{\mathbf x}^{(K+1)})=h(\mathbf x^{(j)})-h(\mathbf x^{(j)} |\bar{\mathbf x}^{(1)},\dots,\bar{\mathbf x}^{(K+1)})~.
\end{align}
Here, $ h(\cdot)$ denotes the Shannon entropy function. Note that the information that adversary can potentially learn about $\mathbf x^j$ by having all $\bar{\mathbf x}^i$'s is fundamentally bounded by  $I(\mathbf x^{(j)} ; \bar{\mathbf x}^{(1)},\dots,\bar{\mathbf x}^{(K+1)})$.  This mutual information in DarKnight can be bounded by the parameters used to blind the data.
\begin{thm}\label{thm:info_leakage1}
Assume that $X^1,\dots,X^K$ are scalars such that $|X^i|\leq C_1$ for all $i$. Suppose $\alpha_{i,j}$'s are standard Gaussian random variables and $R$ is a zero-mean Gaussian random variable with variance $\sigma^2$. Also $\bar X^i$ is defined as
\begin{align}
    \bar X^i=\sum_{j=1}^K \alpha_{j,i} X^j + \alpha_{(K+1),i} R~,\quad i=1,\dots,K+1~.
\end{align}
Then the information leaked from $\bar X^i$'s about $X^j$ is bounded by
\begin{align}\label{eq:infor_bound}
    I\left(X^1,\dots,X^K ; \bar X^1,\dots,\bar X^{(K+1)}\right)\leq \frac{16 K^4 C_1^2}{\sigma^2}~.
\end{align}
\end{thm}
%\vspace{-1mm}
The details of our proof is provided in Appendix A. Note that there is one source of information leakage not considered in the above bound, namely the leakage of inputs from gradients with respect to weight ($\triangledown \mathbf W$). But as we described in Equation \ref{eq:gamma_lin}, we only provide a single model update computed across all the inputs in a batch, which is similar to the state of art secure aggregation mechanisms used to bound such leakage ~\citep{bonawitz2017practical, zhu2019deep}. 


==> 6.Conclusion.tex <==
%\vspace{-9mm}
\section{Conclusion}
\label{sec:con}
%\vspace{-3mm}
This work proposes DarKnight a unified inference and training platform that uses TEE to perform data obfuscation and uses GPU to perform linear operations on obfuscated data. DarKnight uses a novel matrix masking to prevent data exposure. We provide a rigorous proof that bounds DarKnight's information leakage using mutual information. We achieved the privacy of 1 bit leakage on a Megapixel image while using FP operations. 
We evaluated three different models and datasets to demonstrate considerable speedups with provably bounded data privacy leakage and also verifying the computational integrity from GPU. For large DNNs, we observe an average of $12X$ speedup for inference and $5.8X$ speedup for training without accuracy degradation over the baseline fully implemented inside TEE.
